Convex Formulation of Overparameterized Deep Neural Networks

Analysis of over-parameterized neural networks has drawn significant attention in recentyears. It was shown that such systems behave like convex systems under various restrictedsettings, such as for two-level neural networks, and when learning is only restricted locally inthe so-called neural tangent kernel space around specialized initializations. However, there areno theoretical techniques that can analyze fully trained deep neural networks encountered inpractice. This paper solves this fundamental problem by investigating such overparameterizeddeep neural networks when fully trained. We generalize a new technique called neural feature repopulation, originally introduced in (Fang et al., 2019a) for two-level neural networks, to analyze deep neural networks. It is shown that under suitable representations, overparameterized deep neural networks are inherently convex, and when optimized, the system can learn effective features suitable for the underlying learning task under mild conditions. This new analysis is consistent with empirical observations that deep neural networks are capable of learning efficient feature representations. Therefore, the highly unexpected result of this paper can satisfactorily explain the practical success of deep neural networks. Empirical studies confirm that predictions of our theory are consistent with results observed in practice.

==> parts/algorithm.tex <==
\section{Neural Feature Repopulation Algorithm}
\label{sec:algo}



The idea of Neural feature Repopulation can be used to improve the convergence of neural networks, and the process is complementary to the standard SGD procedure. 

%\subsection{Continuous Optimization Procedure}

%\begin{itemize}
%	\item Fix $\rho_0^{(1)}, ..., \rho_0^{(L)}$
%	\item Let $\tilde{\rho}_1^{(\ell)}=\rho_0^{(\ell)}$ 
%	\item Iterate for $t=1,2\ldots$, do
%	\begin{itemize}
%	\item update $\tilde{\u}_t$ by fixing $\tilde{\rho}_t$ and solve
%	\[
%	\tilde{\u}_{t+1} = \arg \min_{\tilde{\u}} J(f(\rho_0, \tilde{\u},\cdot) )
%	+ \tilde{R}(\tilde{\rho}_t,\tilde{\u})
%	\]
%	\item update $\tilde{\rho}_t$ by fixing $\tilde{\u}_{t+1}$ and solve
%	\[
%	\tilde{\rho}_{t+1} =\arg\min_{\tilde{\rho}} \tilde{R}(\tilde{\rho},\tilde{\u}_{t+1}) .
%	\]
%	\end{itemize}
%\end{itemize}


\begin{wraptable}{r}{0.55\textwidth}
\begin{minipage}{1\linewidth}
\begin{algorithm}[H]  
  \caption{Continuous Optimization Procedure}   
  \begin{algorithmic}[1]  
      \STATE {\bfseries Initialization:}  $\tilde{\rho}_1^{(\ell)}=\rho_0^{(\ell)}$ with $\ell=0,\ldots, L$
      \FOR{$t=1$ to T}
      \STATE Update $\tilde{\u}_t$ by fixing $\tilde{\rho}_t$ and solving
	\begin{align}
	\tilde{\u}_{t+1} = \arg \min_{\tilde{\u}} J(f(\rho_0, \tilde{\u};\cdot) )
	+ \tilde{R}(\tilde{\rho}_t,\tilde{\u})\nonumber
	\end{align}
	\STATE Update $\tilde{\rho}_t$ by fixing $\tilde{\u}_{t+1}$ and solving
	\begin{align}
	\tilde{\rho}_{t+1} =\arg\min_{\tilde{\rho}} \tilde{R}(\tilde{\rho},\tilde{\u}_{t+1})\nonumber
	\end{align}
      \ENDFOR
  \STATE {\bfseries Return:} $\tilde{\rho}_{T+1}$ and $\tilde{u}_{T+1}$
  \end{algorithmic}  
\end{algorithm}  
\end{minipage}
\end{wraptable}

Now we can iteratively go from $L$ to $1$ and obtain similar
results. We can now present the characterization of optimal solution via feature
repopulation. 

\begin{theorem}
  The feature repopulation process converges to the optimal solution. 
\end{theorem}








%\subsection{Discrete Feature Repopulation Process}


%\begin{itemize}
%\item Start with initial $(\hat{w}_0,\hat{u}_0)$
%\item Iterate $t=1,2,\ldots$
%\begin{itemize}
%    \item Run multiple steps of SGD with dropouts to obtain updated $(\tilde{w}_t,\tilde{u}_t)$ from $(\hat{w}_{t-1},\hat{u}_{t-1})$
%\item Find $\hat{p}$ to optimize
%\[
%\hat{p}=\arg\min_p \hat{R}(p,\tilde{w}_t,\tilde{u}_t) 
%\]
%with $\hat{R}$ defined in \eqref{eq:reg-im}.
%\item Set initial weights as $(\hat{w}_t,\hat{u}_t)$
%\item For $\ell=1,\ldots, L$, do \\
%Resample the hidden layer $\ell$ for $m^{(\ell)}$ nodes according to $p^{(\ell)}$. Duplicate weights connected to each node before sampling to form the updated weights after sampling.
%  \end{itemize}
%\end{itemize}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../deep"
%%% End:


==> parts/continuousBackup.tex <==
\section{Continuous Deep Neural Networks}\label{sec:continuous-DNNs}

When $m^{(\ell)} \to \infty$, we can define a continuous NN according to the constructed discrete NN.
In this case, the weights $w_j^{(\ell)}$ can be viewed as a real
valued function defined on the weights in the $(\ell-1)$-th layer.  To
this end, we first let $\cZ{0}=\{1,,...,d\}$, and then for all
$\ell \in \{1,...,L\}$, we denote $\cZ{\ell}$ to be  a function
class of real-valued functions defined on $\cZ{\ell-1}$. We  let
$\rho^{(\ell)}(z)$  be a distribution on $\cZ{\ell}$, and let $\rho=\{\rho^{(1)},\ldots,\rho^{(L)}\}$.
Moreover, by convention, we always assume that $\rho^{(0)}$ is the uniform distribution on $\cZ{0}$.
Then the neurons in $\ell$-th layer of the contionuos NN have the following form:
\[
\ff^{(\ell)}(\rho,\z{\ell},x) = h^{(\ell)}\left( \int
  w(\z{\ell},\z{\ell-1}) \ff^{(\ell-1)}(\z{\ell-1},x)
  \rho^{(\ell-1)}(\z{\ell-1}) d \z{\ell-1}\right) 
\]
where $\z{\ell}\in \cZ{\ell}$ and $\ell=1,2,\ldots , L$.
Here 
\[
w(z,z') := z(z') .
\]
Let $\u(\z{L})$ be a real valued function on $\cZ{L}$, then we can define the final output in continuous NN as 
\[
\ff(\rho,\u;x) = \int \u(z^{(L)}) \ff^{(L)}(\rho,z^{(L)},x) \rho^{(L)}(z^{(L)})
d z^{(L)} .
\]
The objective function in continuous NN takes the form of 
\begin{align}
Q(\rho, \u) =& J(f(\rho,\u,\dot)) + R(\rho, \u)\nonumber\\
\mbox{where } R(\rho, \u) =& \sum_{l=1}^L \lambda^{(\ell)}
R^{(\ell)}(\rho) + \lambda^{(\u)} R^{(\u)}(\rho,\u) ,\nonumber
\end{align}
where
%\[
%R^{(\ell)}(\rho)= \int \int |w(\z{\ell},\z{\ell-1})|^{q_\ell} \rho^{(\ell)}(\z{\ell})\rho^{(\ell-1)}(\z{\ell-1})d \z{\ell} d \z{\ell-1}
%\]
\begin{align}
R^{(\ell)}(\rho)=\int r_2\left (\int r_1\big(w (z^{(\ell)}, z^{(\ell-1)})\big)\rho^{(\ell)}(z^{(\ell)})dz^{(\ell)}\right ) \rho^{(\ell-1)}(z^{(\ell-1)})dz^{(\ell-1)}\nonumber
\end{align}
and
\[
R^{(\u)}(\rho,\u) =  \int \|\u(z^{(L)})\|^{q_u}
                 \rho^{(L)}(z^{(L)}) d z^{(L)} .
\]

The connection to discrete version is as follows.
We sample $m^{(\ell)}$ samples $\z{\ell}_i$ from $\rho^{(\ell)}$ for each $\ell$,
and set $w^{(\ell)}_{i,j} = w(\z{\ell}_i,\z{\ell-1}_j)$. 

The following result shows that as $m^{(\ell)} \to \infty$ for all $\ell$, discrete NN converges to the continuous NN. 

\begin{lemma} Suppose that $w^{(\ell)}_{j,k} = w(z^{(\ell)}_j,z^{(\ell-1)}_k), z^{(\ell)}_j \sim \rho^{(\ell)}$ for $\ell=1, ..., L$ and $\u_j = \u(z_j^{(L)})$, then for any $x$,  we have
	\begin{align}
	\lim\limits_{m^{(\ell)}\rightarrow \infty, \ell = 1, ...,L} \hat{f}(x) = f(\rho, u; x).\nonumber
	\end{align}
\end{lemma}
\proof
Firstly, it is obvious that $\hat{f}^{(1)}_j(x){=} f^{(1)}(\rho, z^{(j)}, x)$ holds when $\rho^{(0)}$ is an uniform distribution. 

For $\hat{f}_j^{(2)}(x)$, we have
\begin{align} 
\lim\limits_{m^{(1)}\rightarrow \infty}\hat{f}_j^{(2)}(x) &=\lim\limits_{m^{(1)}\rightarrow \infty} h^{(2)} \left( \frac{1}{m^{(1)}} \sum_{k=1}^{m^{(1)}} w(z^{(2)}_j, z^{(1)}_k) \hat{f}^{(1)}_k(x)\right)\nonumber\\
&=\lim\limits_{m^{(1)}\rightarrow \infty} h^{(2)} \left( \frac{1}{m^{(1)}} \sum_{k=1}^{m^{(1)}} w(z^{(2)}_j, z^{(1)}_k) f^{(1)}(\rho, z^{(1)}_k,x)\right)\nonumber
\end{align}
For $\ell\geq 2$, we assume $\lim\limits_{m^{(\ell-2)}\rightarrow \infty}\ldots\lim\limits_{m^{(1)}\rightarrow \infty} \hat{f}_j^{(\ell-1)}(x) = f^{(\ell-1)}_j(\rho, z^{(\ell-1)}, x)$. Then, we have
\begin{align} 
\lim\limits_{m^{(l)}\rightarrow \infty, l = 1, ...,\ell-1}\hat{f}_j^{(\ell)}(x) &=\lim\limits_{m^{(l)}\rightarrow \infty, l = 1, ...,\ell-1} h^{(\ell)} \left( \frac{1}{m^{(\ell-1)}} \sum_{k=1}^{m^{(\ell-1)}} w(z^{(\ell)}_j, z^{(\ell-1)}_k) \hat{f}^{(\ell-1)}_k(x)\right)\nonumber \\
&=\lim\limits_{m^{(l)}\rightarrow \infty, l = 1, ...,\ell-1} h^{(\ell)} \left( \frac{1}{m^{(\ell-1)}} \sum_{k=1}^{m^{(\ell-1)}} w(z^{(\ell)}_j, z^{(\ell-1)}_k) f^{(\ell-1)}_k(\rho, z^{(\ell-1)}, x)\right)\nonumber \\
&= f^{(\ell)}_j(\rho, z^{(\ell)}, x).\nonumber
\end{align}
Therefore, $\lim\limits_{m^{(\ell)}\rightarrow \infty, \ell = 1, ...,L} \hat{f}_j^{(\ell)}(x) = f^{(\ell)}_j(\rho, z^{(\ell)}, x)$ holds for $\ell = 1, ..., L$. 
For the final output $\hat{f}(x)$, we have
\begin{align}
    \lim\limits_{m^{(\ell)}\rightarrow \infty, \ell = 1, ...,L} \hat{f}(x) &= \lim\limits_{m^{(\ell)}\rightarrow \infty, \ell = 1, ...,L} \frac{1}{m^{(L)}}\sum_{j=1}^{m^{(L)}} u(z_j^{(L)}) \hat{f}_j^{(L)}(x)\nonumber \\
    &=\lim\limits_{m^{(\ell)}\rightarrow \infty, \ell = 1, ...,L} \frac{1}{m^{(L)}}\sum_{j=1}^{m^{(L)}} u(z_j^{(L)}) f_j^{(L)}(x)\nonumber \\
    &= f(\rho, u, x).\nonumber
\end{align} 
This finishes the proof.
\endproof


%\begin{align}
%R^{(\ell)}(p, \rho) &= \int r_2 \left(\int r_1\Big(\frac{w(z^{(\ell)}, z^{(\ell-1)})}{p^{(\ell-1)}(z^{(\ell-1)})}\Big) p^{(\ell-1)}(z^{(\ell-1)}) \rho^{(\ell-1)}(z^{(\ell-1)}) dz^{(\ell-1)}\right) p^{(\ell)}(z^{(\ell)}) \rho^{(\ell)}(z^{(\ell}) dz^{(\ell)}\nonumber\\
%& =  \int r_2 \left(\int r_1\Big(\tilde{w}(z^{(\ell)}, z^{(\ell-1)})\Big) \tilde{\rho}^{(\ell-1)}(z^{(\ell-1)}) dz^{(\ell-1)}\right)  \tilde{\rho}^{(\ell)}(z^{(\ell}) dz^{(\ell)}\nonumber
%\end{align}
%\begin{align}
%R^{(u)}(p,\rho, u) &= \int \frac{|u(z^{(L)})|^2}{p^L(z^{(L)})} \rho^{(L)}(z^{L})dz^{(L)}\nonumber
%\end{align} 
%with 
%\begin{align}
%\tilde{w}(z^{(\ell)}, z^{(\ell-1)}) = \frac{w(z^{(\ell)}, z^{(\ell-1)})}{p^{(\ell-1)}(z^{\ell-1})} \mbox{ and } \tilde{\rho}^{(\ell-1)}(z^{(\ell-1)}) = p^{(\ell-1)}(z^{\ell-1})\rho^{(\ell-1)}(z^{(\ell-1)}),\nonumber
%\end{align}


\subsection{Variance of Discrete Approximation}

The following result shows the variance of such discretization.

\begin{theorem}
Assume the activation functions $h^{(\ell)}(\cdot)$ are smooth: $|\nabla h^{(\ell)}(z)-\nabla h^{(\ell)}(z')| \leq L |z-z'|$ for some $L>0$, where $\nabla h^{(\ell)}(\cdot)$ is the gradient of $h^{(\ell)}(\cdot)$. Define
\[
\hat{g}^{(\ell)}_i(x)=
\frac{1}{m^{(\ell-1)}} \sum_{j=1}^{m^{(\ell-1)}} w^{(\ell)}_{ij} \hat{f}^{(\ell-1)}_j(x) ,
\]
so that $\hat{f}^{(\ell)}_i(x)=h^{(\ell)}(\hat{g}^{(\ell)}_i(x))$. 
Then we have
\begin{align*}
\E_{\xi}  \| \hat{f}(x)-f(x)\|^2 =& \E_{\xi}
\sum_{\ell=2}^{L+1} \frac{1}{(m^{(\ell-1)})^2}
\sum_{j=1}^{m^{(\ell-1)}}  \left(
  \frac{1}{m^{(\ell)}}\sum_{i=1}^{m^{(\ell)}} a_i (x) \big(\hat{f}^{(\ell-1)}_j(x)
  w_{i,j}^{(\ell)} -\hat{g}^{(\ell)}_i(x)\big)\right)^2 \\
 & + O\left( \sum_{\ell} (m^{(\ell)})^{-1.5}  \right) ,
\end{align*}
where $a_i(x)= (\partial \hat{f}(\cdot)/\partial \hat{g}^{(\ell)}_i(\cdot))(x)$, and 
$\xi$ denotes a random sampled discrete architecture underlying $\hat{f}(\cdot)$ from its continuous version $f(\cdot)$.
\label{thm:variance}
\end{theorem}

If one can learn good feature representations, then the variance of discrete approximation is small. This will lead to a regularization condition that determines how good feature representation. Specifically if we assume that $|a_i(x)\hat{f}^{(\ell-1)}_j(x)|$ is bounded, then in order to minimize variance, we can minimize the following regularization:
\[
R^{(\ell)}(w^{(\ell)})
= \frac{1}{m^{\ell-1}} 
\sum_{j=1}^{m^{(\ell-1)}}  \left(
  \frac{1}{m^{(\ell)}}\sum_{i=1}^{m^{(\ell)}}
  |w_{i,j}^{(\ell)}| \right)^2 ,
\]
which corresponds to picking $r_1(w)=|w|$ and $r_2(w)=w^2$ in \eqref{eq:reg}.

%\textbf{My question:} whether a realvalued function is appropriate for modeling the weights? For example, when $z^{l}_i, z^$


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../deep"
%%% End:

